OntoScene, A Logic-based Scene Interpreter: Implementation and Application in the Rock Art Domain

We present OntoScene, a framework aimed at understanding the semantics of visual scenes starting from the semantics of their elements and the spatial relations holding between them. OntoScene exploits ontologies for representing knowledge and Prolog for specifying the interpretation rules that domain experts may adopt, and for implementing the SceneInterpreter engine. Ontologies allow the designer to formalize the domain in a reusable way, and make the system modular and interoperable with existing multiagent systems, while Prolog provides a solid basis to define complex rules of interpretation in a way that can be affordable even for people with no background in Computational Logics. The domain selected for experimenting OntoScene is that of prehistoric rock art, which provides us with a fascinating and challenging testbed. Under consideration in Theory and Practice of Logic Programming (TPLP)

==> backg.tex <==
\section{Background}\label{sec:background}

OntoScene is meant to be used inside a JADE MAS and heavily exploits the tools that JADE offers to integrate ontologies in the MAS. Giving for granted some familiarity of the reader with knowledge representation in general and with ontologies in particular\footnote{The reader may find an introduction to computational ontologies in \cite{guarino2009ontology}, the specification of the OWL Web Ontology Language in \cite{mcguinness2004owl}, and information on Prot\'eg\'e on the official web site, \url{https://protege.stanford.edu/}, accessed on January 2019.}, in this section we provide a brief introduction to JADE and to the way ontologies are supported therein. We also provide references to the JPL Library for interfacing SWI-Prolog and Java, and to the JTS Topology Suite we used to compute spatial relationships among elements in a scene.   

\paragraph{JADE.}
%
JADE (Java Agent DEvelopment Framework, \cite{bellifemine2007developing}) is a Java-based software platform that supports the development of agents and MASs thanks to a Graphical User Interface and tools supporting the MAS debugging and deployment phases. JADE MASs can be distributed across machines in a way which is fully transparent to the developer. The minimal system requirement is the the Java run time environment or JDK, version 5.

\paragraph{Ontologies in JADE.}
%
JADE helps developers in achieving semantic interoperability between agents thanks to a simple and fast way to exploit ontologies directly inside the platform and the agents: agents can exchange messages referring to a shared ontology, and then rely on the Jade Ontology management offered by the ContentManager class.
The developer may use an ontology to formalize what the agents knows (Concepts and Predicates) and can do (Actions), and share this ontology among the agents: in this way, knowledge is modelled outside the agents boosting modularity and reuse, and the content of messages is based on a shared ontology, facilitating interactions and simplifying the serialization phase that is then demanded to the JADE platform.

The three types of objects considered when creating an ontology for JADE are:
\begin{itemize}
\item Predicates: boolean expressions describing something about the agent environment or its beliefs.
\item Concepts: structured objects describing the elements of the world, and their relationships.
\item Agent actions: special Concepts modeling what an agent can do and can be requested to do with a message.
\end{itemize}

If two agents share the same ontology, one agent can request the other to perform an Action, and can receive an answer containing the Action results, which will be a Concept, a Predicate, or a list of them.

%Manually Creating this types of Java representation of an ontology (which is usually already written in an ontology language) can be done, but is complex and long above all if the ontology is complex: furthermore, every time the ontology changes, its Java representation must be updated, and above all, often developers are not the same people who design the ontology, and both the involved figures are usually not abel to write both in OWL (or similar language) and in Java. Consequently, designers and expert of the domains should focus on modeling the ontology in a language, and developers should focus on managing this ontology in Java for Jade. 


To allow developers to automatically generate a Java  representation  of  an OWL  ontology  coherent  with the JADE requirements, the tool OntologyBeanGenerator\footnote{\url{https://protegewiki.stanford.edu/wiki/OntologyBeanGenerator}, accessed on January 2019.} can be adopted. The latest version of OntologyBeanGenerator available on the official web site is the 4.1, including a basic ontology modeling the over mentioned concepts: domain specific concepts must be added as subclasses of Concept, Predicate and Agent, and then the tool will provide a Java representation of the ontology, directly usable by JADE.

Given some limitations of that version, we developed OntologyBeanGenerator 5.0 \cite{WOA18} as a new Prot\'eg\'e plugin\footnote{We asked and obtained a written consent from the author of OntologyBeanGenerator, Chris van Aart, to extend the original source code.}.
%
%\paragraph{OntologyBeanGenerator 5.0.}
%\label{sec:BeanGenerator2}
%
%To support the designer in the automatic exportation of an OWL ontology into a Java format that JADE is directly able to exploit, we developed the OntologyBeanGenerator 5.0 . 
OntologyBeanGenerator 5.0 (OBG5.0 in the sequel) has been developed with three goals in mind: correcting some bugs of OntologyBeanGenerator 4.1; adding the methods and exceptions management directly inside the ontology; and producing an additional output to support the OntoScene framework.


The main improvements of OBG5.0 w.r.t. OntologyBeanGenerator 4.1 are:
\begin{itemize}
\item Addition of a new tab called Java Method Mapper to manage the methods creation and exportation: the purpose of the new tab is to offer the designer of the ontology a way to directly add methods to the Java version of the ontology: in the previous version, the only way was to add a property and consequently to get the setter and getter automatically. 
%This is mainly foreseen if we want to add methods that cannot be mapped in a setter/getter of a specific field. %These methods are saved in an external XML file which is loaded by the tab and overwritten when exporting the ontology;
\item Exception management: methods are allowed to raise Exceptions. To do this, a specific ontology to be imported has been created.
\item Correction of some bugs that were present in the ontology generation stage. %: now the ontology correctly extends BeanOntology;
%\item Automatic import of the Default Implementation of the classes in the Java Ontology;
\item Possibility to export classes in a Prolog format: {\bf DANY}
\end{itemize}


\paragraph{The JPL Library.} JPL\footnote{\url{http://www.swi-prolog.org/packages/jpl/},  accessed on January 2019.} can be used to embed SWI-Prolog in Java as well as for embedding Java in SWI-Prolog. In both setups it provides a reentrant bidirectional interface. 

\verb|jpl_call(+Object, +Method, +Params, -Result)|
    unifies \texttt{Result} with a JPL reference to (or value of) the result of calling the named method of \texttt{Object} with \texttt{Params}, e.g. \verb|jpl_call(F, setVisible, [@(true)], _)|.
    

\paragraph{The JTS Suite.} 
The JTS Topology Suite (JTS\footnote{\url{https://locationtech.github.io/jts/},  accessed on January 2019.}) is an open source Java software library that provides an object model for planar geometry together with a set of fundamental geometric functions. In OntoScene, it was used as a general-purpose library providing algorithms in computational geometry, to implement some useful topological relations. 

To make an example of combined use of JPL+JTS, if \texttt{GR} is a reference to an object implementing geometric relations in JTS, 
\verb|jpl_call(GR, contains, [BB1, BB2], @(true))| succeeds if the JTS method \texttt{contains} called on \texttt{BB1} (the bounding box of one image) and \texttt{BB2} (the bounding box of another image), returns \texttt{true}. 
In a similar way, we may have \verb|jpl_call(GR, overlap, [BB1, BB2], @(true)))|, \verb|jpl_call(GR, group, [JavaBBs, 0.5], @(true))|, \verb|jpl_call(GR, vertical, [BB2, BB1, 'up'], @(true))|, \verb|jpl_call(GR, near, [BB1, BB2, 0.5], @(true))| with their intuitive meaning, better explained in Section \ref{subsec:geomrel}.


